Words, Concepts, and the Geometry of Analogy

This paper presents a geometric approach to the problem of modelling the relationship between words and concepts, focusing in particular on analogical phenomena in language and cognition. Grounded in recent theories regarding geometric conceptual spaces, we begin with an analysis of existing static distributional semantic models and move on to an exploration of a dynamic approach to using high dimensional spaces of word meaning to project subspaces where analogies can potentially be solved in an online, contextualised way. The crucial element of this analysis is the positioning of statistics in a geometric environment replete with opportunities for interpretation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{39}
\providecommand{\publicationstatus}{Kartsaklis, D., Lewis, M. and Rimell, L. (Eds):\\2016 Workshop on Semantic Spaces at the Intersection of\\NLP, Physics and Cognitive Science (SLPCS'16)\\
EPTCS 221, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.221.5}{10.4204/EPTCS.221.5}}

